Dynamic Random Choice

I study dynamic random utility with finite choice sets and exogenous total menu variation, which I refer to as stochastic utility (SU). First, I characterize SU when each choice set has three elements. Next, I prove several mathematical identities for joint, marginal, and conditional Block--Marschak sums, which I use to obtain two characterizations of SU when each choice set but the last has three elements. As a corollary under the same cardinality restrictions, I sharpen an axiom to obtain a characterization of SU with full support over preference tuples. I conclude by characterizing SU without cardinality restrictions. All of my results hold over an arbitrary finite discrete time horizon.

==> Old/2_RU.tex <==
\section{Random Utility}
\label{sec:ru}
Before introducing SU, I provide a brief overview of RU and its axiomatization. Let $X$ be a finite choice set, and let $\mathcal{M}:=2^{X}\backslash\{\emptyset\}$ be the set of all nonempty menus. Given a (exogenously-chosen) menu $A \in \mathcal{M}$, the agent makes a choice $x \in A$. The agent's choice data for all nonempty menus is encoded in the following primitive:

\begin{definition}
A \textbf{stochastic choice function} is a mapping $\rho: \mathcal{M} \rightarrow \Delta(X)$ satisfying $\text{supp }\rho(A) \subseteq A$ for all $A \in \mathcal{M}$.
\end{definition}

Stochastic choice functions must satisfy $\text{supp }\rho(A) \subseteq A$ because the agent can only pick from choices within the menu. As in \cite{SC}, I use $\rho$ to denote a stochastic choice function and $\rho(x,A)$ to denote the probability that $\rho(A)$ assigns $x$. Let $P$ be the set of strict preference relations over $X$, and let $C(x,A):=\big\{\succ \in P: x \succ A\backslash\{x\}\big\}$.\footnote{$P$ can also be viewed as the set of permutations of $X$. The notation $x \succ A\backslash\{x\}$ denotes $x \succ y \ \forall \ y \in A\backslash\{x\}$.} Observe that $\{C(x,A)\}_{x \in A}$ form a partition of $P$.

\begin{definition}
$\mu \in \Delta(P)$ is a \textbf{random utility (RU) representation} of $\rho$ if $\rho(x,A)=\mu\big(C(x,A)\big)$ for all $x \in A \in \mathcal{M}$.
\end{definition}

In the deterministic case, it is well-known that a choice function can be represented by a strict preference relation if and only if it satisfies Sen's $\alpha$ condition, as shown in \cite{sen1971choice}. I will now state the analogous axiomatization of RU, first for $|X|\leq 3$ and second for any finite $X$.

\begin{axiom}
$\rho$ satisfies \textbf{regularity} if $\rho(x,A) \geq \rho(x,B)$ for all $x \in A \subseteq B \in \mathcal{M}$.
\end{axiom}

As stated in \cite{SC}, regularity serves as the stochastic analog of Sen's $\alpha$. Regularity is necessary for RU because $C(x,A) \supseteq C(x,B)$ for all $x \in A \subseteq B$. In particular, when the choice set is of size three or less, regularity characterizes RU.

\begin{lemma}[\textbf{\cite{block1959random}}]
Suppose $|X| \leq 3$. $\rho$ has a RU representation if and only if it satisfies regularity.
\end{lemma}

If the choice set satisfies these cardinalities, \cite{SC} shows that the RU representation is also unique. For higher cardinalities, a stronger axiom is needed to characterize RU.

\begin{definition}[\textbf{\cite{chambers2016revealed}}]
For any $A \subsetneq X$ and $x \in A^C$, define their \textbf{Block-Marschak sum} to be
\begin{align*}
    M_{x,A}:=\sum_{B \supseteq A^C} (-1)^{|B\backslash A^C|} \rho(x,B)
\end{align*}
\end{definition}

\begin{axiom}[\textbf{\cite{chambers2016revealed}}]
$\rho$ satisfies \textbf{Block-Marschak nonnegativity} if $M_{x,A} \geq 0$ for all $x \in A^C \neq \emptyset$.
\end{axiom}

\begin{lemma}[\textbf{\cite{block1959random}; \cite{falmagne1978representation}}]
$\rho$ has a RU representation if and only if it satisfies Block-Marschak nonnegativity.
\end{lemma}

With these two axiomatizations in hand, I turn to the dynamic model.

==> Old/4_Corollaries.tex <==
\section{Corollaries}
\label{sec:cor}

\subsection{SU with Full Support}
As shown by \cite{fishburn1998stochastic}, for arbitrary finite $X$ RU representations need not be unique. This also implies that, in general, SU representations need not be unique.\footnote{To see this, let $\mu_1,\mu_1' \in \Delta(P_1)$ be distinct RU representations of $\rho_1$, and let $\mu_2 \in \Delta(P_2)$. Let $\mu=\mu_1 \times \mu_2$, $\mu'=\mu_1' \times \mu_2$: it follows that $\mu\big(C(x_2,A_2)|C(x_1,A_1)\big)=\mu_2\big(C_2(x_2,A_2)\big)=\mu'\big(C(x_2,A_2)|C(x_1,A_1)\big)$.} Indeed, sometimes it may be desirable to represent $\boldsymbol{\rho}^2$ using a SU representation with full support over $P_1 \times P_2$.\footnote{The existence of such a representation is equivalent to the existence of a distribution over $\mathbb{R}^{X_1} \times \mathbb{R}^{X_2}$ with positive density.}

\begin{definition}
$\mu \in \Delta(P_1 \times P_2)$ has \textbf{full support} if $\mu(\succ_1,\succ_2)>0$ for all $(\succ_1,\succ_2) \in P_1 \times P_2$.
\end{definition}

It turns out that characterizing this case requires only a slightly stronger version of \textbf{Axiom 3}.

\begin{axiom}
$\boldsymbol{\rho}^2$ satisfies \textbf{stochastic Block-Marschak positivity} if $M_{x_1,A_1;x_2,A_2}>0$ for each $t=1,2$ and $x_t \in A_t^C \neq \emptyset$.
\end{axiom}

\begin{corollary}
$\boldsymbol{\rho}^2$ has a SU representation with full support if and only if it satisfies stochastic Block-Marschak positivity and marginal consistency.\footnote{Analogously, $\rho$ has a RU representation with full support if and only if it satisfies the strict version of \textbf{Axiom 2}. The proof proceeds analogously to the proof of this corollary.}
\end{corollary}

Observe that stochastic Block-Marschak positivity is necessary because probability measures with full support assign strictly positive probability to all nonempty events.

\subsection{More Periods}
\textcolor{red}{I am currently working on extending \textbf{Theorem 1} to more than two periods with multiperiod versions of both axioms.} Fix $n>2$. The primitive is now the vector 
\begin{align*}
    \boldsymbol{\rho}^n:=\big(\rho_1,\{\rho_2(\cdot|h_1)\}_{h_1 \in \mathcal{H}_1},\ldots,\{\rho_n(\cdot|h_{n-1})\}_{h_{n-1} \in \mathcal{H}_{n-1}}\big)
\end{align*}
where $\mathcal{H}_1:=\{(A_1,x_1): \rho_1(x_1,A_1)>0\}$ and $\mathcal{H}_t:=\{(A_t,x_t;h_{t-1}) \in \mathcal{M}_t \times X_t \times \mathcal{H}_{t-1}: \rho_t(x_t,A_t|h_{t-1})>0\}$ for all $t>1$. As before, WLOG let $\rho_t(\cdot,A_t|A_{t-1},x_{t-1};\cdots;A_1,x_1) \in \Delta(A_t)$ be an arbitrary probability distribution if $\rho_{t'}(x_{t'},A_{t'}|A_{t'-1},x_{t'-1};\cdots;A_1,x_1)=0$. Define $P_t,C_t(x_t,A_t),C(x_t,A_t)$ as before. Given $t>1$ and $h_t=(A_t,x_t;h_{t-1})$, define $C(h_t):=C(x_t,A_t) \cap C(h_{t-1})$.

\begin{definition}[\textbf{\cite{SC}}]
$\mu \in \Delta\big(\bigtimes_{t=1}^n P_t\big)$ is a ($n$-period) \textbf{stochastic utility (SU) representation} of $\boldsymbol{\rho}^n$ if $\rho_1(x_1,A_1)=\mu\big(C(x_1,A_1)\big)$ for all $x_1 \in A_1 \in \mathcal{M}_1$ and $\rho_t(x_t,A_t|h_{t-1})=\mu\big(C(x_t,A_t)|C(h_{t-1})\big)$ for all $x_t \in A_t \in \mathcal{M}_t$ and $h_{t-1} \in \mathcal{H}_{t-1}$.
\end{definition}

Now, we generalize the axioms. Let $(\boldsymbol{x},\boldsymbol{A}):=(x_t,A_t)_{t=1}^n$ and $(\boldsymbol{x}_{-t},\boldsymbol{A}_{-t})=(x_{t'},A_{t'})_{t'=1,t'\neq t}^n$. Let $\boldsymbol{A}^C=(A_t^C)_{t=1}^n$, and say $\boldsymbol{B}\geq\boldsymbol{A} \iff B_t \supseteq A_t$ for each $t=1,\ldots,n$. Let $j(\boldsymbol{x},\boldsymbol{A})=\rho_1(x_1,A_1)\prod_{t=2}^n \rho_t(x_t,A_t|A_{t-1},x_{t-1};\ldots,A_1,x_1)$.

\begin{axiom}
$\boldsymbol{\rho}^n$ satisfies ($n$-period) \textbf{stochastic Block-Marschak nonnegativity} if
\begin{align*}
    M_{(\boldsymbol{x},\boldsymbol{A})}:=\sum_{\boldsymbol{B} \geq \boldsymbol{A}^C} (-1)^{\sum_{t=1}^n |B_t\backslash A_t^C|} j(\boldsymbol{x},\boldsymbol{B}) \geq 0
\end{align*}
for all $(\boldsymbol{x},\boldsymbol{A})$ satisfying $x_t \in A_t^C \neq \emptyset$ for each $t=1,\ldots,n$.
\end{axiom}

\begin{axiom}
$\boldsymbol{\rho}^n$ satisfies ($n$-period) \textbf{marginal consistency} if for any $(\boldsymbol{x},\boldsymbol{A})$ and $t=1,\ldots,n-1$,
\begin{align*}
    P(\boldsymbol{x}_{-t},\boldsymbol{A}_{-t};A_t):=\sum_{x_t \in A_t} j(\boldsymbol{x}_{-t},\boldsymbol{A}_{-t};x_t,A_t)
\end{align*}
is invariant in $A_t$.
\end{axiom}

\begin{corollary}[\textcolor{red}{\textbf{Conjecture}}]
$\boldsymbol{\rho}^n$ has a SU representation if and only if it satisfies stochastic Block-Marschak nonnegativity and marginal consistency.
\end{corollary}

As before, to prove \textbf{Corollary 2} it will be helpful to have the following generalization of \textbf{Proposition 3} in hand.

\begin{corollary}[\textcolor{red}{\textbf{Conjecture}}]
$\mu$ is a SU representation of $\boldsymbol{\rho^n}$ if and only if $\mu\big(E(\boldsymbol{x},\boldsymbol{A})\big)=M_{(\boldsymbol{x},\boldsymbol{A})}$ for all $(\boldsymbol{x},\boldsymbol{A})$ satisfying $x_t \in A_t^C \neq \emptyset$ for each $t=1,\ldots,n$,
where
\begin{align*}
    E(\boldsymbol{x},\boldsymbol{A}):=\big\{(\succ_1,\ldots,\succ_n) \in \bigtimes_{t=1}^n P_t: A_t \succ_t x_t \succ_t A_t^C\backslash\{x_t\}, \ t=1,\ldots,n\big\}
\end{align*}
\end{corollary}

==> Old/6_SuppApp.tex <==
\subsection{Proof of Corollary 2, Forwards Direction}


\subsection{Proof of Corollary 2, Backwards Direction}
Since the proof proceeds analogously to the proof of \textbf{Theorem 1}, we will omit some of the details. See this for reference.



\subsection{Proof of Corollary 3}
\begin{proof}
First, we prove a generalization of \textbf{Proposition 1}.

\begin{claim}
For all $(\boldsymbol{x},\boldsymbol{A}$ satisfying $x_t \in A_t^C \neq \emptyset$,
\begin{align*}
    \rho_1(x_1,A_1^C)\prod_{t=2}^n \rho_t(x_t,A_t^C|A_{t-1}^C,x_{t-1};\cdots;A_1^C,x_1)=\sum_{\boldsymbol{D} \leq \boldsymbol{A}} M_{(\boldsymbol{x},\boldsymbol{D})}
\end{align*}
\end{claim}

Let $(L,\leq)$ be the product poset of $\{(2^{X_t},\subseteq)\}_{t=1}^n$ and define
\begin{align*}
    f(\boldsymbol{B}):=(-1)^{\sum_{t=1}^n |B_t|-|A_t^C|} \rho_1(x_1,B_1)\prod_{t=2}^n \rho_t(x_t,B_t|B_{t-1},x_{t-1};\cdots;B_1,x_1)
\end{align*}
and $F(\boldsymbol{D})=\sum_{\boldsymbol{B} \geq \boldsymbol{D}} f(\boldsymbol{B})$. By \textbf{Lemmas 2, 3, and 4}, 
\begin{align*}
    \rho_1(x_1,A_1^C)\prod_{t=2}^n \rho_t(x_t,A_t^C|A_{t-1}^C,x_{t-1};\cdots;A_1^C,x_1)=\sum_{\boldsymbol{B} \geq \boldsymbol{A}^C} (-1)^{\sum_{t=1}^n |B_t|-|A_t^C|} F(\boldsymbol{B})=\sum_{\boldsymbol{D} \leq \boldsymbol{A}} M_{(\boldsymbol{x},\boldsymbol{D})}
\end{align*}
since $(-1)^{\sum_{t=1}^n |D_t^C|-|A_t^C|} F(\boldsymbol{D}^C)=M_{(\boldsymbol{x},\boldsymbol{D})}$. \\ \\
Forwards direction: suppose $\mu$ is a SU representation of $\boldsymbol{\rho}^n$. By \textbf{Lemma 2},
\begin{align*}
    \rho_1(x_1,A_1^C)\prod_{t=2}^n \rho_t(x_t,A_t^C|A_{t-1}^C,x_{t-1};\cdots;A_1^C,x_1)=\sum_{\boldsymbol{B} \geq \boldsymbol{A}^C} \mu\big(E(\boldsymbol{x},\boldsymbol{B}^C)\big) \\
    \implies \mu\big(E(\boldsymbol{x},\boldsymbol{A})\big)=M_{(\boldsymbol{x},\boldsymbol{A})}
\end{align*}
Backwards direction: suppose $\mu\big(E(\boldsymbol{x},\boldsymbol{A})\big)=M_{(\boldsymbol{x},\boldsymbol{A})}$ for all $(\boldsymbol{x},\boldsymbol{A})$ satisfying $x_t \in A_t^C \neq \emptyset$. By \textbf{Claim 6},

\end{proof}

==> Old/SU.tex <==
\section{Stochastic Utility}\label{sec:su}

\subsection{Preliminaries}
Now, I examine the dynamic analog of \textbf{Section}'s choice environment: dynamic riskless stochastic choice over arbitrary finite choice sets. Although I prove some of this section's results for arbitrary finite time periods in the \textbf{Appendix}, I state them for two time periods for ease of exposition. Index these time periods by $t \in \{1,2\}$. For each $t$, let $X_t$ be a finite choice set, $\mathcal{M}_t$ be the set of nonempty subsets of $X_t$, and $\Delta(X_t)$ be the set of probability distributions over $X_t$. Let a \textit{(static) SCF} be a function satisfying \textbf{Definition}.

\begin{definition}
A \textbf{dynamic stochastic choice function (DSCF)} is a pair $(\rho_1,\rho_2)$ such that:
\begin{enumerate}
    \item $\rho_1: \mathcal{M}_1 \rightarrow \Delta(X_1)$ is a SCF.
    \item $\rho_2: \mathcal{H} \times \mathcal{M}_2 \rightarrow \Delta(X_2)$ maps each \textbf{history} $h \in \mathcal{H}$ to the SCF $\rho_2(\cdot|h)$, where
    $$\mathcal{H}:=\{(A_1,x_1) \in \mathcal{M}_1\times X_1: \rho_1(x_1,A_1)>0\}$$
\end{enumerate}
\end{definition}

I take the DSCF $(\rho_1,\rho_2)$ as primitive, which is generated by repeated trials of the following form: the agent exogenously receives $A_1$, chooses $x_1 \in A_1$, exogenously receives $A_2$, and chooses $x_2 \in A_2$. Over many trials, her period-1 choices are aggregated into $\rho_1$. Since every period-2 choice is preceded by some period-1 choice that occurs with positive probability, her period-2 choices following history $(A_1,x_1)$ are aggregated into the \textit{conditional SCF} $\rho_2(\cdot|A_1,x_1)$. For $(A_1,x_1)$ such that $\rho_1(x_1,A_1)=0$, let $\rho_2(\cdot,A_2|A_1,x_1) \in \Delta(A_2)$ be any probability distribution. Thus, for any menus $A_1 \in \mathcal{M}_1$ and $A_2 \in \mathcal{M}_2$, my augmented DSCF admits a well-defined joint distribution over $A_1\times A_2$, where $(x_1,x_2)$ is assigned probability $\rho_2(x_2,A_2|A_1,x_1)\rho_1(x_1,A_1)$.

As before, let $P_t$ be the set of strict preference relations over $X_t$. For $x_t \in A_t$, define $C_t(x_t,A_t):=\big\{\succ_t \ \in P_t: x_t \succ_t A_t\backslash\{x_t\}\big\}$ and $C(x_t,A_t):=C_t(x_t,A_t) \times P_{-t}$.\footnote{Let $\{t,-t\}=\{1,2\}$.}

\begin{definition}[\cite{SC}]
$\mu \in \Delta(P_1 \times P_2)$ is a (two-period) \textbf{stochastic utility (SU) representation} of $\boldsymbol{\rho}^2$ if $\rho_1(x_1,A_1)=\mu\big(C(x_1,A_1)\big)$ for all $x_1 \in A_1 \in \mathcal{M}_1$ and $\rho_2(x_2,A_2|A_1,x_1)=\mu\big(C(x_2,A_2)|C(x_1,A_1)\big)$ for all $x_2 \in A_2 \in \mathcal{M}_2$ and $(A_1,x_1) \in \mathcal{H}$.
\end{definition}

If $\mu$ is a SU representation of $\boldsymbol{\rho}^2$, note that its marginal over $P_1$ is a RU representation of $\rho_1$ and its conditional $\mu\big(\cdot|C(x_1,A_1)\big)$ is a RU representation of $\rho_2(\cdot|A_1,x_1)$ for $(A_1,x_1) \in \mathcal{H}$.

\begin{definition}
For each $t=1,2$ and $x_t \in A_t^C \neq \emptyset$, define their \textbf{joint Block-Marschak sum} to be
\begin{align*}
    M_{x_1,A_1;x_2,A_2}:=\sum_{B_2 \supseteq A_2^C} \sum_{B_1 \supseteq A_1^C} (-1)^{|B_1\backslash A_1^C|+|B_2\backslash A_2^C|} \rho_2(x_2,B_2|B_1,x_1)\rho_1(x_1,B_1)
\end{align*}
and their \textbf{joint upper edge set}\footnote{Joint upper edge sets are a generalization of what \cite{chambers2016revealed} define as \textit{upper contour sets}.} to be
\begin{align*}
    E(x_1,A_1;x_2,A_2):=\{(\succ_1,\succ_2) \in P_1 \times P_2: A_t \succ_t x_t \succ_t A_t^C\backslash \{x_t\}, \ t=1,2\}
\end{align*}
\end{definition}

\subsection{Axiomatization}
\begin{axiom}
$\boldsymbol{\rho}^2$ satisfy \textbf{stochastic Block-Marschak nonnegativity} if $M_{x_1,A_1;x_2,A_2} \geq 0$ for each $t=1,2$ and $x_t \in A_t^C \neq \emptyset$.
\end{axiom}

As its name suggests, \textbf{Axiom 3} serves as the two-period analog of \textbf{Axiom 2}. Unlike the static case, \textbf{Axiom 3} is not sufficient, and another axiom that enforces consistency between periods is needed to complete the characterization.

\begin{axiom}
$\boldsymbol{\rho}^2$ satisfy \textbf{marginal consistency}\footnote{In \cite{SC}, this is stated as the \textit{LTP axiom}.} if
\begin{align*}
    P(x_2,A_2;A_1):=\sum_{x_1 \in A_1} \rho_2(x_2,A_2|A_1,x_1)\rho_1(x_1,A_1)
\end{align*}
is invariant in $A_1$ for all $x_2 \in A_2 \in \mathcal{M}_2$.
\end{axiom}

The main result of this paper is that \textbf{Axioms 1 and 2} characterize two-period SU:

\begin{theorem}
$\boldsymbol{\rho}^2$ has a SU representation if and only if it satisfies stochastic Block-Marschak nonnegativity and marginal consistency.
\end{theorem}

The full proof of \textbf{Theorem 1} is in \textbf{Section 5}, but I will provide a sketch here. First, I will state several helpful propositions. \textbf{Propositions 1 and 2}\footnote{\textbf{Proposition 1} is the two-period analog of \textbf{Lemma 7.4.I} in \cite{chambers2016revealed}, while \textbf{Proposition 2} is a partial generalization of \textbf{Lemma 7.4.II} in the same book.} serve as useful identities for the joint Block-Marschak sums, and \textbf{Proposition 3}\footnote{This is the two-period analog of \textbf{Proposition 7.3.} in \cite{chambers2016revealed}.} characterizes SU representations as probability measures that assign each joint upper edge set its corresponding joint Block-Marschak sum. 

\begin{proposition}
For each $t=1,2$ and $x_t \in A_t^C \neq \emptyset$
\begin{align*}
    \rho_2(x_2,A_2^C|A_1^C,x_1)\rho_1(x_1,A_1^C)=\sum_{B_2 \subseteq A_2} \sum_{B_1 \subseteq A_1} M_{x_1,B_1;x_2,B_2}
\end{align*}
\end{proposition}

\begin{proposition}
For any $x_1 \in A_1^C \neq \emptyset$ and $\emptyset \subsetneq A_2 \subsetneq X_2$
\begin{align*}
    \sum_{x_2 \in A_2^C} M_{x_1,A_1;x_2,A_2}=\sum_{y_2 \in A_2} M_{x_1,A_1;y_2,A_2\backslash\{y_2\}}
\end{align*}
\end{proposition}

\begin{proposition}
$\mu$ is a SU representation of $\boldsymbol{\rho}^2$ if and only if $\mu\big(E(x_1,A_1;x_2,A_2)\big)=M_{x_1,A_1;x_2,A_2}$ for each $t=1,2$ and $x_t \in A_t^C \neq \emptyset$.
\end{proposition}

To prove the forwards direction of \textbf{Theorem 1}, note that \textbf{Proposition 3} immediately implies that stochastic Block-Marschak nonnegativity is necessary, since probability measures assign nonnegative values to all events.\footnote{Analogous reasoning provides intuition for why Block-Marschak nonnegativity is necessary for static RU.} Marginal consistency is necessary because of the Law of Total Probability. With \textbf{Proposition 3} in hand, it follows that to prove the backwards direction, it suffices to construct a probability measure $\mu \in \Delta(P_1 \times P_2)$ that assigns each joint upper edge set its corresponding joint Block-Marschak sum. I do this in \hyperref[sec:app]{\textbf{Section 5}} via the following steps:\footnote{The proof strategy for this direction is adapted from the proof of the static case in \cite{chambers2016revealed}.}
\begin{enumerate}
    \item Using marginal consistency, prove the period-1 equivalent of \textbf{Proposition 2}.
    \item Using stochastic Block-Marschak nonnegativity, recursively define a ``partial measure" $\nu$. $\nu$ is ``partial" in the following sense: it is not defined on all subsets of $P_1 \times P_2$, but rather on pairs of subsets called $t$-\textit{cylinders}.
    \item Verify that $\nu$ satisfies two crucial additivity properties over the pairs of $t$-cylinders.
    \item Use both additivity properties to define a probability measure $\mu$ that is an extension of $\nu$, and verify that $\mu$ assigns each joint upper edge set its corresponding joint Block-Marschak sum.
\end{enumerate}

\subsection{Axiomatization for $\boldsymbol{|X_1|=|X_2|=3}$}
At lower choice set cardinalities, we can restate stochastic Block-Marschak nonnegativity as a simpler axiom.

\begin{axiom}
$\boldsymbol{\rho}^2$ satisfies \textbf{stochastic regularity} if for each $t=1,2$ and $x_t \in A_t \subseteq B_t$,
\begin{align*}
    \frac{\rho_1(x_1,A_1)}{\rho_1(x_1,B_1)} \geq \frac{\rho_2(x_2,A_2|B_1,x_1)-\rho_2(x_2,B_2|B_1,x_1)}{\rho_2(x_2,A_2|A_1,x_1)-\rho_2(x_2,B_2|A_1,x_1)}
\end{align*}
\end{axiom}
Stochastic regularity is necessary because $x_t \in A_t \subseteq B_t$ for each $t=1,2$ implies
\begin{align*}
    C(x_1,A_1) \cap \bigg(C(x_2,A_2)\backslash C(x_2,B_2)\bigg) \supseteq C(x_1,B_1) \cap \bigg(C(x_2,A_2)\backslash C(x_2,B_2)\bigg)
\end{align*}
When $|X_1|=|X_2|=3$ and marginal consistency holds, it is also sufficient.

\begin{proposition}
Suppose $|X_1|=|X_2|=3$. $\boldsymbol{\rho}^2$ has a unique SU representation if and only if it satisfies stochastic regularity and marginal consistency.
\end{proposition}



